Application of the third RIT binary black hole simulations catalog to parameter estimation of gravitational waves signals from the LIGO-Virgo O1/O2 observational runs

Using exclusively the 777 full numerical waveforms of the third Binary Black Holes RIT catalog, we reanalyze the ten black hole merger signals reported in LIGO/Virgo's O1/O2 observation runs. We obtain binary parameters, extrinsic parameters, and the remnant properties of these gravitational waves events which are consistent with, but not identical to previously presented results. We have also analyzed three additional events (GW170121, GW170304, GW170727) reported in Venumadhav et al. 2019, and found closely matching parameters. We finally assess the accuracy of our waveforms with convergence studies applied to O1/O2 events and found them adequate for current estimation of parameters.

==> aligned-additionalGWEvents.tex <==
\begin{table*}
  \caption{(Top) Doing a GPR fit to find the highest $\ln{\cal L}$ from the nonprecessing simulations. Parameter estimation of
    the mass ratio $q$, the individual spins $a_1$ and $a_2$, the total mass of the system in the detector frame, $M_t$ and the effective spin variable
    $S_{hu}$, at the maximum of $\ln{\cal L}$ and its $90\%$ confidence ranges.
(Bottom) Parameter estimation of
    the final black hole mass $m_f$, spin $a_f$, and its recoil velocity $v_f$,
    and the Luminosity $p_L$, waveform frequency $p_O$ at the maximum amplitude $p_A$, at the maximum of $\ln{\cal L}$ and its $90\%$ confidence ranges from the nonprecessing simulations.
\label{tab:aligned-additional}}
\begin{ruledtabular}
\begin{tabular}{lcccccc}
  Event/$f_{min}$ & Max($\ln{\cal L}$) & $q^{max}$ & $a_1^{max}$ & $a_2^{max}$ & $M_t^{max}$ & $S_{hu}^{max}$ \\
\hline
GW170121 & & & & & &  \\
20Hz & Range & & & & &  \\
GW170727 & & & & & &  \\
20Hz & Range & & & & &  \\
\hline\hline
 Event & $m_f^{max}$ & $a_f^{max}$ & $v_f^{max}$ & $p_L^{max}$ & $p_O^{max}$ & $p_A^{max}$\\
\hline
GW170121 & & & & & &  \\
20Hz & Range & & & & &  \\
GW170727 & & & & & &  \\
20Hz & Range & & & & &  \\
\end{tabular}
\end{ruledtabular}
\end{table*}


==> extrinsic-Figs.tex <==
\begin{figure*}
\includegraphics[angle=0,width=1.95\columnwidth]{figs/GW150914_H1_RIT_strain.png}
\includegraphics[angle=0,width=1.95\columnwidth]{figs/GW150914_L1_RIT_strain.png}
  \caption{Reconstruction of NR simulation with extrinsic 
            parameters given in Table~\ref{tab:extrinsic} compared to GW150914.
  \label{fig:GW150914_reconstruction}}
\end{figure*}

\begin{figure*}
\includegraphics[angle=0,width=1.95\columnwidth]{figs/GW151012_H1_RIT_strain.png}
\includegraphics[angle=0,width=1.95\columnwidth]{figs/GW151012_L1_RIT_strain.png}
  \caption{Reconstruction of NR simulation with extrinsic 
            parameters given in Table~\ref{tab:extrinsic} compared to GW151012.
  \label{fig:GW151012_reconstruction}}
\end{figure*}

\begin{figure*}
\includegraphics[angle=0,width=1.95\columnwidth]{figs/GW151226_H1_RIT_strain.png}
\includegraphics[angle=0,width=1.95\columnwidth]{figs/GW151226_L1_RIT_strain.png}
  \caption{Reconstruction of NR simulation with extrinsic 
            parameters given in Table~\ref{tab:extrinsic} compared to GW151226.
  \label{fig:GW151226_reconstruction}}
\end{figure*}

\begin{figure*}
\includegraphics[angle=0,width=1.95\columnwidth]{figs/GW170104_H1_RIT_strain.png}
\includegraphics[angle=0,width=1.95\columnwidth]{figs/GW170104_L1_RIT_strain.png}
  \caption{Reconstruction of NR simulation with extrinsic 
            parameters given in Table~\ref{tab:extrinsic} compared to GW170104.
  \label{fig:GW170104_reconstruction}}
\end{figure*}

\begin{figure*}
\includegraphics[angle=0,width=1.95\columnwidth]{figs/GW170608_H1_RIT_strain.png}
\includegraphics[angle=0,width=1.95\columnwidth]{figs/GW170608_L1_RIT_strain.png}
  \caption{Reconstruction of NR simulation with extrinsic 
            parameters given in Table~\ref{tab:extrinsic} compared to GW170608.
  \label{fig:GW170608_reconstruction}}
\end{figure*}

\begin{figure*}
\includegraphics[angle=0,width=1.95\columnwidth]{figs/GW170729_H1_RIT_strain.png}
\includegraphics[angle=0,width=1.95\columnwidth]{figs/GW170729_L1_RIT_strain.png}
  \caption{Reconstruction of NR simulation with extrinsic 
            parameters given in Table~\ref{tab:extrinsic} compared to GW170729.
  \label{fig:GW170729_reconstruction}}
\end{figure*}

\begin{figure*}
\includegraphics[angle=0,width=1.95\columnwidth]{figs/GW170809_H1_RIT_strain.png}
\includegraphics[angle=0,width=1.95\columnwidth]{figs/GW170809_L1_RIT_strain.png}
\includegraphics[angle=0,width=1.95\columnwidth]{figs/GW170809_V1_RIT_strain.png}
  \caption{Reconstruction of NR simulation with extrinsic 
            parameters given in Table~\ref{tab:extrinsic} compared to GW170809.
  \label{fig:GW170809_reconstruction}}
\end{figure*}

\begin{figure*}
\includegraphics[angle=0,width=1.95\columnwidth]{figs/GW170814_H1_RIT_strain.png}
\includegraphics[angle=0,width=1.95\columnwidth]{figs/GW170814_L1_RIT_strain.png}
\includegraphics[angle=0,width=1.95\columnwidth]{figs/GW170814_V1_RIT_strain.png}
  \caption{Reconstruction of NR simulation with extrinsic 
            parameters given in Table~\ref{tab:extrinsic} compared to GW170814.
  \label{fig:GW170814_reconstruction}}
\end{figure*}

\begin{figure*}
\includegraphics[angle=0,width=1.95\columnwidth]{figs/GW170818_H1_RIT_strain.png}
\includegraphics[angle=0,width=1.95\columnwidth]{figs/GW170818_L1_RIT_strain.png}
\includegraphics[angle=0,width=1.95\columnwidth]{figs/GW170818_V1_RIT_strain.png}
  \caption{Reconstruction of NR simulation with extrinsic 
            parameters given in Table~\ref{tab:extrinsic} compared to GW170818.
  \label{fig:GW170818_reconstruction}}
\end{figure*}

\begin{figure*}
\includegraphics[angle=0,width=1.95\columnwidth]{figs/GW170823_H1_RIT_strain.png}
\includegraphics[angle=0,width=1.95\columnwidth]{figs/GW170823_L1_RIT_strain.png}
  \caption{Reconstruction of NR simulation with extrinsic 
            parameters given in Table~\ref{tab:extrinsic} compared to GW170823.
  \label{fig:GW170823_reconstruction}}
\end{figure*}


